A Tailored Pre-Training Model for Task-Oriented Dialog Generation

The recent success of large pre-trained language models such as BERT and GPT-2 has suggested the effectiveness of incorporating language priors in downstream dialog generation tasks. However, the performance of pre-trained models on the dialog task is not as optimal as expected. In this paper, we propose a Pre-trained Role Alternating Language model (PRAL), designed specifically for task-oriented conversational systems. We adopted (Wu et al., 2019) that models two speakers separately. We also design several techniques, such as start position randomization, knowledge distillation, and history discount to improve pre-training performance. We introduce a task-oriented dialog pretraining dataset by cleaning 13 existing data sets. We test PRAL on three different downstream tasks. The results show that PRAL performs better or on par with state-of-the-art methods.

==> figures/res_table_MultiWOZ.tex <==

\begin{table}[t]
\centering
\tablestyle{0.1pt}{1.25}
\begin{tabular}{l|cc|ccc}
 \toprule
 \textbf{\multirow{2}*{Model}} & \multicolumn{2}{c|}{\textbf{Supervision}} &  \textbf{\multirow{2}*{BLEU-4}} & \textbf{\multirow{2}*{Inform}}  & \textbf{\multirow{2}*{Success}}  \\ 
 & Dialog State & Dialog Act &&& \\
 \hline 
 Human & - & - & -  & 0.989 & 0.965 \\ \hline 
 Baseline & $\checkmark$ &  $\times$ & 18.9  & 0.825  & 0.729  \\
 HDSA &  $\checkmark$ &  $\checkmark$ & \textbf{23.6}  & \textbf{0.877} &  0.734 \\
 LaRL &  $\checkmark$ &  $\times$ & 12.8  & 0.828  & \textbf{0.792}  \\ \hline
 ARDM &  $\times$ &  $\times$ & 20.6 &  0.874 &  0.728 \\
 \modelname{} &  $\times$ &  $\times$ & 21.6  & 0.875  & 0.742  \\
 \bottomrule
\end{tabular}
\caption{Results on MultiWOZ dataset}
\label{table:mutliWOZ}
\end{table}

==> figures/res_table_camrest676.tex <==

\begin{table}[t]
\centering
\tablestyle{3.2pt}{1.25}
\begin{tabular}{lcc}
 \toprule
 \textbf{Model} & \textbf{BLEU-4} & \textbf{Success. F1}  \\ \hline
 Sequicity & 21.4 & 0.852 \\
 Sequicity (w/o RL) & 22.9 & 0.821 \\
 GPT-2-finetune  & 21.8 & 0.851 \\
 DialoGPT & 25.2  & 0.861 \\
 ARDM  & 26.2 & 0.864  \\ \hline
 \modelname{} & \textbf{27.3} & \textbf{0.870}\\
 \hspace{2mm} - w/o discount factor & 27.0 & 0.867 \\
 \hspace{2mm} - w/o random position & 26.6 & 0.869 \\
 \hspace{2mm} - w/o constrain & 25.0 & 0.865  \\
 \hspace{2mm} - small constrain & 26.9 & 0.869  \\
 \bottomrule
\end{tabular}
\caption{Results on CamRest676 dataset.}
\label{tab:camres}
\end{table}

==> figures/res_table_persuasion.tex <==
\begin{table*}[t]
\centering
\tablestyle{4.1pt}{1.21}
\begin{tabular}{l|ccc|cccccc}
 \toprule
      & Perplexity $\downarrow$  & BLEU-1 $\uparrow$   &  BLEU-2 $\uparrow$  &  Fluency & Logic  & Coherence  & Diversity & Overall & Avg.Donation $\uparrow$
      \\ \hline
 ARDM & \textbf{10.1}  & 16.5  & 6.44  & 0.39  & 0.41  & 0.37 & 0.27 & 0.18 & 0.62  \\
 \modelname{} & 10.3  & \textbf{17.3}
 & \textbf{10.9}  & \textbf{0.61}  & \textbf{0.59}  & \textbf{0.63} & \textbf{0.73} & \textbf{0.82} & \textbf{0.99}  \\
 \bottomrule
\end{tabular}
\caption{Automatic Evaluation and Human Evaluation Results}
\label{table:persuasion}
\end{table*}



\begin{comment}
\begin{table}[h]
\centering
\begin{tabular}{lccc}
 \toprule
 & & ARDM &  \modelname{} \\ \hline
 & Perplexity & &   \\
 & BLEU-1 & &   \\
 & BLEU-2 & &   \\ \hline
 & Fluent & &   \\
 & Logic & &   \\
 & Coherence & &  \\ 
 & Diversity & &   \\
 & Overall & &   \\
 & Donation Average & &  \\
 \bottomrule
\end{tabular}
\caption{PersuasionforGood, Automatic Evaluation and Human Evaluation Results}
\label{table:persuasion}
\end{table}
\end{comment}

==> figures/table_backup.tex <==
\begin{table*}[h]
    \centering
    \resizebox{.9\textwidth}{!}{
        \begin{tabular}{l|c|cc}
        \toprule
        Model &  \quad BLEU-4 & Success. F1\\
       
        \midrule
        GPT-2-finetune  & 21.8 & 0.851 \\
        \midrule
        ARDM  & 26.7 & 0.864  \\
        \midrule
        \modelname{} & \textbf{27.3} & \textbf{0.870}\\
        \modelname{} w/o random position & 26.6 & 0.869 \\
        \modelname{} w/o constrain & 25.0 & 0.865  \\
        \modelname{} small constrain & 26.2 & 0.869  \\
        \modelname{} w/o discount factor &  & \\
        \bottomrule
        \end{tabular}
    }
    \caption{Results on CamRest676 dataset.
    % We evaluate the situation when the training set only contains 50\% data (200 examples).
    }
    \label{tab:camres}
\end{table*}


\subsection{MultiWOZ}
\begin{table*}[h]
    \centering
    
    \begin{tabular}{l|cc|c|c|c}
    \toprule
     \multirow{2}*{Model}& \multirow{2}*{Inform } & \multirow{2}*{Success } & \multirow{2}*{BLEU-4} \\  & & & \\
    \midrule
    Human & 0.989 & 0.965 & -  \\
    \midrule
    Baseline &  0.825 & 0.729 & 18.9 \\  
    % Sequicity &  $\checkmark$ & $\times$ & 86.6 & 71.6 & 16.8 \\
    HDSA & \textbf{0.877} & 0.734 & \textbf{23.6} \\
    % SFN + RL &  $\checkmark$ & $\checkmark$ & 82.7 & 72.1 & 16.3 \\
    LaRL  &0.828 & \textbf{0.792} & 12.8 \\
    \midrule
    ARDM & 0.874 & 0.728 & 20.6  \\
    \modelname{} & 0.875 & 0.742 & 21.6  \\
    \bottomrule
    \end{tabular}
    
    \caption{Results on MultiWOZ. 
    Supervision denotes whether a model leverages dialog state or/and dialog act annotations. 
    All models use the ground truth dialog state for database search.
    \modelname{} without supervision from annotation can still achieve comparable results.
    }
    \label{tab:multiwoz}
\end{table*}

\begin{table*}[h]
        \centering
        \resizebox{.95\textwidth}{!}{
        \begin{tabular}{l|ccc|c|c|c}
        \toprule
        & Perplexity $\downarrow$ & BLEU-1 $\uparrow$ & BLEU-2 $\uparrow$ & logic & coherence & Average $\uparrow$ \\ 
        \midrule
        % {\fontsize{11}{7.2}\selectfont TransferTransfo} & 19.9 & 17.0 & 8.57 &0 & 0  & 0.538 \\ 
        %\midrule
        ARDM & \textbf{10.1} & 16.5 & 6.44  & 0 & 0  & 0 \\
        \modelname{} & 10.3 &  \textbf{17.3} & \textbf{10.9}  & 0 & 0 & 0 \\
        \bottomrule
        \end{tabular}
        }
        \caption{Automatic Evaluation and Human Evaluation Results}
        \label{tab:persuasion_automatic}
\end{table*}
